Rogue Signs: Deceiving Traffic Sign Recognition with Malicious Ads and Logos

We propose a new real-world attack against the computer vision based systems of autonomous vehicles (AVs). Our novel Sign Embedding attack exploits the concept of adversarial examples to modify innocuous signs and advertisements in the environment such that they are classified as the adversary's desired traffic sign with high confidence. Our attack greatly expands the scope of the threat posed to AVs since adversaries are no longer restricted to just modifying existing traffic signs as in previous work. Our attack pipeline generates adversarial samples which are robust to the environmental conditions and noisy image transformations present in the physical world. We ensure this by including a variety of possible image transformations in the optimization problem used to generate adversarial samples. We verify the robustness of the adversarial samples by printing them out and carrying out drive-by tests simulating the conditions under which image capture would occur in a real-world scenario. We experimented with physical attack samples for different distances, lighting conditions and camera angles. In addition, extensive evaluations were carried out in the virtual setting for a variety of image transformations. The adversarial samples generated using our method have adversarial success rates in excess of 95% in the physical as well as virtual settings.

==> future_work.tex <==
While our traffic sign recognition system performs well in spite of its simplicity, more robust traffic sign recognition systems exist in the literature, especially ones based on neural networks that can simultaneously handle both detection and classification in real time  such as Faster R-CNN \cite{Ren15frcnn} and YOLOv2 \cite{Redmon16yolo}. We are currently exploring attacks on these systems as well.

Further, we are exploring methods to secure the computer vision systems of self-driving cars against these attacks. One plausible solution is to deploy adversarially trained neural networks \cite{goodfellow2014explaining,tramer2017ensemble,madry_towards_2017} which have been shown to be more robust than standard neural networks against virtual adversarial samples. However, it is unclear if these will be effective against \signembedding attacks, a direction we are exploring. Further, since the \lentprinting attack does not rely on the phenomenon of adversarial examples, we propose the exploration of authenticated road signs to boost the safety of self-driving cars. \arjun{@Arsalan add content here} 

% Our choice for measuring visibility of the perturbation is chosen as \todo{cite: papers that use L1 norm} where $L_1$ norm is used. However, we understand that the choice is, to a certain degree, arbitrarily, and we do not argue that it is the best measurement. Rather, we encourage future works to conduct users study to determine a more appropriate proxy to measure perceptibility of the perturbation.
